Nonparametric Regression, Confidence Regions and Regularization

In this paper we offer a unified approach to the problem of nonparametric regression on the unit interval. It is based on a universal, honest and non-asymptotic confidence region which is defined by a set of linear inequalities involving the values of the functions at the design points. Interest will typically centre on certain simplest functions in that region where simplicity can be defined in terms of shape (number of local extremes, intervals of convexity/concavity) or smoothness (bounds on derivatives) or a combination of both. Once some form of regularization has been decided upon the confidence region can be used to provide honest non-asymptotic confidence bounds which are less informative but conceptually much simpler.

==> shaperegfig.tex <==
\section{Figures}
\quad\\
% \begin{figure}[ht]
%   \centering
%   \psfig{file=wave05_15.ps,angle=270,height=5.7cm,width=12cm}
%   \caption{ The figure shows the sine curve, the sine curve with a
%     bump and the reconstructions of both using wavelets as described
%     in the text. The sample size is $2^{15}=32768$ and both curves
%     were contaminated with exactly the same noise. \label{wave05_15}} 
% \end{figure}
%\afterpage{\clearpage}
\begin{figure}[ht]
  \centering
 \psfig{file=wave05_16.ps,angle=270,height=5cm,width=12cm}
  \psfig{file=ts05_16.ps,angle=270,height=5cm,width=12cm}
  \caption{ Reconstructions of a noisy sine curve and sine curve with
    bump. The upper panel shows the wavelet reconstructions and the
    lower panel the taut string reconstructions as described in the
    text. The sample size is $2^{16}=65536$ and all curves were
    contaminated with exactly the same noise.  \label{wave05_16}} 
\end{figure}
%\afterpage{\clearpage}
%\newpage

\begin{figure}[ht]
  \centering
  \psfig{file=wave05_20.ps,angle=270,height=5cm,width=12cm}
  \psfig{file=ts05_20.ps,angle=270,height=5cm,width=12cm}
  \caption{  Reconstructions of a noisy sine curve and
    sine curve with bump on the interval $[0.2,\,0.4].$  The upper
    panel shows the wavelet reconstructions and the lower panel the
    taut string reconstructions as described in the text. The sample
    size is $2^{20}=1048576$ and all curves  were contaminated with
    exactly the same noise.  \label{wave05_20}} 
\end{figure}

%\newpage
\begin{figure}[htb]
  \centering
  \psfig{file=hwts11.ps,angle=270,width=12cm,height=6cm}
  \psfig{file=hwts13.ps,angle=270,width=12cm,height=6cm}
  \psfig{file=hwts12.ps,angle=270,width=12cm,height=6cm}
  \caption{ The first 200 data points of data
    generated according to (\ref{sequmod}) with $\sigma=1$ (top
    panel) and the taut string reconstruction (centre panel) and the
    Haar wavelet reconstruction (bottom panel). The function 
    $f_n$ is as given by (\ref{fn1}) with $n=1024,
    \gamma_n=0.005, \Gamma_n=0.01$ and $\delta_n=4.5.$  \label{hwts1}}
\end{figure}

%\newpage


% \begin{figure}[htb]
%   \centering
%   \psfig{file=misetshwpckloc.ps,angle=270,height=8cm,width=12cm}
%   \caption{ The upper panel shows the RMISE of the Haar wavelet
%     reconstruction as a function of the position of the peaks as
%     described in the text. The lower panel shows the corresponding
%     result for the taut string reconstruction. 
%   \label{misetshwpckloc}}
% \end{figure}





\begin{figure}[htb]
  \centering
  \psfig{file=rmisetswv.ps,angle=270,height=6cm,width=12cm}
  \caption{ $\log(\text{RMISE})$ plotted against
    $\log_2(n)$ for the Haar wavelets (upper points) and for the taut string
    (lower points). The parameter values are as given by (\ref{valpar}). The sample
    sizes range from 2048 to 4194304. \label{rmisetswv}}
\end{figure}



% \begin{figure}[htb]
%   \centering
%   \psfig{file=stndrdrmisetswv.ps,angle=270,height=6cm,width=12cm}
%   \caption{ The figure shows the standardized RMISE plotted against
%     $\log_2(n)$ for the Haar wavelets (black) and for the taut string
%     (red). The standardization for the Haar wavelets is $0.1RMISE
%     \times(n\Gamma_n/\log(1/\Gamma_n))$ and for the taut string $RMISE
%     \times(n\Gamma_n/\log(n\Gamma_n)).$ The parameter values are as given by
%     (\ref{valpar}). The sample sizes range from 2048 to
%     4194304. \label{stndrdrmisetswv}} 
% \end{figure}

% \begin{figure}[htb]
%   \centering
%   \psfig{file=tshwrecon.ps,angle=270,height=6cm,width=12cm}
%   \caption{ The figure shows function $f_n$ (black), the Haar wavelet
%     reconstruction (blue) and the taut string reconstruction (red) on
%     an interval $I_{n,k}^c$ as given by (\ref{definkc}). The sample
%   size is $n=2^{18}=262144$ and the length of $I_{nk}^c$ is 200. The
%   values of the parameters for $f_n$ are as given by (\ref{valpar}).
%   \label{tshwrecon}}
% \end{figure}



%\newpage
\begin{figure}[htb]
  \centering
  \psfig{file=FIGmintv0doppler.ps,angle=270,height=6cm,width=12cm}
  \psfig{file=FIGmintv1doppler.ps,angle=270,height=6cm,width=12cm}
  \caption{ Minimization of $TV({\tilde f}_n)$  (upper panel) and
    $TV({\tilde f}_n^{(1)})$ (lower panel)  subject to ${\tilde f}_n \in {\mathcal
      A}_n$ for a noisy Doppler function. \label{dopplermintv}}
\end{figure}

\newpage
\begin{figure}
  \centering
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sin.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sinwv.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}\\
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sind1.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sinwvd1.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}\\
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sind2.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sinwvd2.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}\\
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sind3.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sinwvd3.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}\\
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sind4.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}
  \begin{minipage}[b]{.5\linewidth}
    \psfig{file=FIGminabsd4sinwvd4.ps,angle=270,height=3cm,width=5.5cm}
  \end{minipage}
  \caption{ The reconstruction of a noisy sine function $Y(t)=\sin(4\pi t)+0.1Z(t)$
    and its first four derivatives from a sample of size $n=1024$. The lines
    show from top to bottom the reconstruction of the function itself and its
    first four derivatives. The left column shows the reconstructions obtained by 
    minimizing  $\Vert {\tilde f}_n^{(4)}\Vert.$ The right column shows the
    wavelet reconstructions using the Daubechies least-asymmetric orthonormal
    compactly supported wavelet with 10 vanishing moments. Superimposed are
    the corresponding derivatives of $\sin(4\pi t)$. 
\label{dsin4pid0:4}}
\end{figure}

\newpage






\begin{figure}[htb]
  \centering
  \psfig{file=mintv2mon.ps,angle=270,height=6cm,width=12cm}
  \caption{ The minimization of the total variation of the second
    derivative with  (solid line) and without (dashed line) the shape 
    constraints  derived from the taut string. The solution
    subject to the shape constraints was also forced to assume the
    same value at the local maximum as the taut string solution.
 \label{mintv2mon}}
\end{figure}

\begin{figure}[htb]
  \centering
  \psfig{file=expfnbndsinc.ps,angle=270,height=6cm,width=12cm}
\psfig{file=expfnbndscnvx.ps,angle=270,height=6cm,width=12cm}
  \caption{ The function $f(t)=\exp(5t)$ degraded with $N(0,25)$ noise
    together with monotone confidence bounds (upper panel) and convex
    confidence bounds (lower panel). The three lower bounds in the
    upper panel are derived from (\ref{nondecrlow}), (\ref{fastlowerincr}) and
    (\ref{superfastlowerincr}) and the 
corresponding upper bounds are (\ref{nondecrupp}), (\ref{fastupperincr}) and
(\ref{superfastupperincr}). The lower bounds for the lower panel are
(\ref{lowcnvx}), (\ref{fastlowercnvx}) and (\ref{superfastlowercnvx})
and the corresponding upper bounds (\ref{uppcnvx}), (\ref{fastuppercnvx}) and
(\ref{superfastuppercnvx}) \label{expfnbndsinccnvx}}
\end{figure}

% \begin{figure}[htb]
%   \centering
  
%   \caption{ The figure shows generated by (\ref{expdata}) together
%     with the lower bounds ( and the
% corresponding upper bounds . The $\sigma$ in the above bounds was
% replaced by $\sigma_n$ of (\ref{sigman}). \label{expfnbndscnvx}}
% \end{figure}

% \newpage
% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLcbdav_sin_maxloc.ps,angle=270,height=6cm,width=12cm}
%   \caption{ The figure shows the confidence bounds corresponding to
%     two different choices for the position of the local maximum. 
% \label{EXMPLcbdav_sin_maxloc}}
% \end{figure}


\begin{figure}[htb]
  \centering
  \psfig{file=EXMPLcbdav_sin_maxint.ps,angle=270,height=6cm,width=12cm}
  \psfig{file=EXMPLcbdav_sin_2_maxautots.ps,angle=270,height=6cm,width=12cm} 
  \caption{ Confidence bounds without (upper panel) and with (lower
    panel) the specification of the precise positions of the local extreme
    values. The positions in the lower panel are the default choices
    obtained from the taut string reconstruction.
    \label{EXMPLcbdav_sin_2_maxautots}}
\end{figure}

% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLcbdav_sin_maxint.ps,angle=270,height=6cm,width=12cm}
%   \caption{ The figure shows the confidence bounds corresponding to
%     an interval of possible positions of the local maximum. 
% \label{EXMPLcbdav_sin_maxint}}
% \end{figure}
% \newpage

% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLcbdav_sin_2_maxautots.ps,angle=270,height=6cm,width=12cm}  
%   \caption{ The figure shows the confidence bounds corresponding to
%     the taut string default choices for the positions of the local
%     extremes. \label{EXMPLcbdav_sin_2_maxautots}}
% \end{figure}


% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLcbdav_sin_2_cvx_auto_tv1.ps,angle=270,height=6cm,width=12cm}
%    \caption{ The figure shows the result of minimizing the total  
%     variation of the first derivative. 
%   \label{EXMPLcbdav_sin_2_cvx_auto_tv1}} 
% \end{figure}
%\newpage

\begin{figure}[htb]
  \centering
  \psfig{file=EXMPLcbdav_sin_2_cvx_auto.ps,angle=270,height=6cm,width=12cm}  
  \psfig{file=EXMPLcbdav_sin_2_cvx_auto_mon.ps,angle=270,height=6cm,width=12cm} 
  \caption{ Confidence bounds with default choices for the intervals of
    convexity/concavity (upper panel) and combined confidence
    bounds for default choices of intervals of monotonicity and
    convexity/concavity. \label{EXMPLcbdav_sin_2_cvx_auto}}
\end{figure}



% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLcbdav_sin_2_cvx_auto.ps,angle=270,height=6cm,width=12cm}  
%   \caption{ The figure shows the confidence bounds corresponding to
%     the default choices for the intervals of convexity and concavity.
%   \label{EXMPLcbdav_sin_2_cvx_auto}} 
% \end{figure}

% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLcbdav_sin_2_cvx_auto_mon.ps,angle=270,height=6cm,width=12cm}  
%   \caption{ The figure shows the confidence bounds for the data of
%     Figures \ref{EXMPLcbdav_sin_2_maxautots} and 
%     \ref{EXMPLcbdav_sin_2_cvx_auto} with both the monotone and
%     convexity/concavity constraints
%     imposed. \label{EXMPLcbdav_sin_2_cvx_auto_mon}}  
% \end{figure}

\newpage

\begin{figure}[htb]
  \centering
  \psfig{file=EXMPL_sin_cb1.ps,angle=270,height=6cm,width=12cm}  
  \psfig{file=EXMPLsin_cb_all.ps,angle=270,height=6cm,width=12cm} 
  \psfig{file=EXMPL_sin_cb_fast.ps,angle=270,height=6cm,width=12cm}  
  \caption{Smoothness confidence bounds for $f \in {\mathcal
      F}_n=\{f:\Vert {\tilde f}_n^{(2)}\Vert _{\infty} \le K\}$ for
    data generated according to (\ref{standmod}) with $f(t)=\sin(4\pi
    t),\,\sigma=0.2$ and $n=500.$ 
    The top panel shows the function which minimizes  $\Vert {\tilde
      f}_n^{(2)}\Vert _{\infty}$. The minimum is  115 compared with
    $16\pi^2=157.9$ for $f(t)$. For this value of $K$ the bounds are
    degenerate. The centre panel shows the confidence bounds for $K=
    136.5, \,157.9$ and $315.8$  The bottom panel shows the  
  corresponding fast bounds  (\ref{lbfastsmooth}) and
  (\ref{ubfastsmooth}) for the same values of $K.$ 
%   \caption{ The figure shows data generated according to
%     (\ref{standmod}) with $f(t)=\sin(4\pi t),\,\sigma=1$ and $n=500$ together
%     with the function $f^*_n$ 
%     which minimizes $\Vert {\tilde f}_n^{(2)}\Vert _{\infty}$ amongst
%     all functions ${\tilde f}_n \in {\mathcal A}_n.$ The value  $\Vert
%     {\tilde f}_n^{(2)}\Vert _{\infty}$ is 115.0465 compared with
%     $16\pi^2=157.9137$ for $\Vert f^{(2)}\Vert_\infty.$
    \label{EXMPL_sin_cb1}}
\end{figure}

% \begin{figure}[htb]
%   \centering
%   \psfig{file=EXMPLsin_cb_all.ps,angle=270,height=6cm,width=12cm} 
%   \psfig{file=EXMPL_sin_cb_fast.ps,angle=270,height=6cm,width=12cm}  
% \caption{The second panel shows the same data of  Figure \ref{EXMPL_sin_cb1}
%     together with the bounds based on $K=136.5,\,\,157.9$ and 315.8.
%     The lower panel shows the same data with the fast bounds using the same values for $K$.}
%  \caption{ The figure shows data of  Figure \ref{EXMPL_sin_cb1}
%    together with the bounds based on $K=136.5,\,\,157.9$ and 315.8.
% \label{EXMPLsin_cb_all}}   
%\end{figure}


%\newpage
%\begin{figure}[htb]
%  \centering
%  \psfig{file=EXMPL_sin_cb_fast.ps,angle=270,height=6cm,width=12cm}  
%  \caption{ The figure shows data of Figure \ref{EXMPL_sin_cb1}
%    together with the fast bounds of (\ref{lbfastsmooth}) and
%    (\ref{lbfastsmooth}) for the same values of $K$ as for Figure. 
%    \label{EXMPL_sin_cb_fast}}   
%\end{figure}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "shapereg_ims"
%%% End: 

